Photo Stylistic Brush: Robust Style Transfer via Superpixel-Based Bipartite Graph

With the rapid development of social network and multimedia technology, customized image and video stylization has been widely used for various social-media applications. In this paper, we explore the problem of exemplar-based photo style transfer, which provides a flexible and convenient way to invoke fantastic visual impression. Rather than investigating some fixed artistic patterns to represent certain styles as was done in some previous works, our work emphasizes styles related to a series of visual effects in the photograph, e.g. color, tone, and contrast. We propose a photo stylistic brush, an automatic robust style transfer approach based on Superpixel-based BIpartite Graph (SuperBIG). A two-step bipartite graph algorithm with different granularity levels is employed to aggregate pixels into superpixels and find their correspondences. In the first step, with the extracted hierarchical features, a bipartite graph is constructed to describe the content similarity for pixel partition to produce superpixels. In the second step, superpixels in the input/reference image are rematched to form a new superpixel-based bipartite graph, and superpixel-level correspondences are generated by a bipartite matching. Finally, the refined correspondence guides SuperBIG to perform the transformation in a decorrelated color space. Extensive experimental results demonstrate the effectiveness and robustness of the proposed method for transferring various styles of exemplar images, even for some challenging cases, such as night images.

==> Lourvre1-2.tex <==
\def\hs{-0.3cm}
\def\height{3.1cm}
\begin{figure*}[htbp]
	\begin{center}
		{
			\subfigure[Input]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre-2.png}
			}
			\hspace{\hs}
			\subfigure[L$\alpha\beta$]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre_CIE_1-2.png}
			}
			\hspace{\hs}
			\subfigure[Harmonization]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre_harmonization_1-2.png}
			}
			\hspace{\hs}
			\subfigure[Landmark]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre_Landmark_1-2.png}
			}
			\\
			\vspace{-3mm}
			
			\subfigure[Reference]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre-1.png}
			}	
			\hspace{\hs}		
			\subfigure[NeutralArt]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre_NeutralArt_1-2.png}
			}
			\hspace{\hs}
			\subfigure[SuperMatch]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre_SuperMatch_1-2.png}
			}
			\hspace{\hs}
			\subfigure[SuperBig]{
				\includegraphics[height=\height,clip]{./Images/Lourvre1-2/Louvre_SuperBig_Modified_1-2.png}
			}
		}
	\end{center}
	\vspace{-7mm}
	
	\caption{ Visual comparisons of style transfer from (a) to (e) among different algorithms.}
	\label{fig:Lourvre1}
\end{figure*}

==> Roma-1.tex <==

\def\height{2.3cm}
\begin{figure*}[htbp]
	\begin{center}
		{
			\subfigure[Input]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma-1.png}
			}
			\subfigure[L$\alpha\beta$]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma_CIE_1-2.png}
			}
			\subfigure[Harmonization]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma_harmonization_1-2.png}
			}
			\subfigure[Landmark]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma_Landmark_1-2.png}
			}
			\\
			\subfigure[Reference]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma-2.png}
			}			
			\subfigure[NeutralArt]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma_NeutralArt_1-2.png}
			}
			\subfigure[SuperMatch]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma_SuperMatch_1-2.png}
			}
			\subfigure[SuperBig]{
				\includegraphics[height=\height,clip]{./Images/Roma1-2/roma_SuperBig_1-2.png}
			}
		}
	\end{center}
	\vspace{-2mm}
	\caption{ Visual comparisons of style transfer among different algorithms.}
	\label{fig:roma1-2}
\end{figure*}


==> Roma-2.tex <==

\def\height{2.3cm}
\begin{figure*}[htbp]
	\begin{center}
		{
			\subfigure[Input]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma-2.png}
			}
			\subfigure[L$\alpha\beta$]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma_CIE_2-1.png}
			}
			\subfigure[Harmonization]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma_harmonization_2-1.png}
			}
			\subfigure[Landmark]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma_Landmark_2-1.png}
			}
			\\
			\subfigure[Reference]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma-1.png}
			}			
			\subfigure[NeutralArt]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma_NeutralArt_2-1.png}
			}
			\subfigure[SuperMatch]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma_SuperMatch_2-1.png}
			}
			\subfigure[SuperBig]{
				\includegraphics[height=\height,clip]{./Images/Roma2-1/roma_SuperBig_2-1.png}
			}
		}
	\end{center}
	
	\caption{ Visual comparisons of style transfer among different algorithms.}
	\label{fig:roma1-2}
\end{figure*}

==> Roma-3.tex <==

\def\height{2.3cm}
\begin{figure*}[htbp]
	\begin{center}
		{
			\subfigure[Input]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma-3.png}
			}
			\subfigure[L$\alpha\beta$]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_CIE_3-4.png}
			}
			\subfigure[Harmonization]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_harmonization_3-4.png}
			}
			\subfigure[Landmark]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_Landmark_3-4.png}
			}
			\\
			\subfigure[Reference]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma-4.png}
			}			
			\subfigure[NeutralArt]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_NeutralArt_3-4.png}
			}
			\subfigure[SuperMatch]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_SuperMatch_3-4.png}
			}
			\subfigure[SuperBig]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_SuperBig_3-4.png}
			}
		}
	\end{center}
	
	\caption{ Visual comparisons of style transfer among different algorithms.}
	\label{fig:roma3-4}
\end{figure*}

==> Roma-4.tex <==

\def\height{2.3cm}
\begin{figure*}[htbp]
	\begin{center}
		{
			\subfigure[Input]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma-3.png}
			}
			\subfigure[L$\alpha\beta$]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_CIE_3-4.png}
			}
			\subfigure[Harmonization]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_harmonization_3-4.png}
			}
			\subfigure[Landmark]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_Landmark_3-4.png}
			}
			\\
			\subfigure[Reference]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma-4.png}
			}			
			\subfigure[NeutralArt]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_NeutralArt_3-4.png}
			}
			\subfigure[SuperMatch]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_SuperMatch_3-4.png}
			}
			\subfigure[SuperBig]{
				\includegraphics[height=\height,clip]{./Images/Roma3-4/Roma_SuperBig_3-4.png}
			}
		}
	\end{center}
	
	\caption{ Visual comparisons of style transfer among different algorithms.}
	\label{fig:roma3-4}
\end{figure*}

==> Taj-2.tex <==

\def\height{2.5cm}
\begin{figure*}[htbp]
	\begin{center}
		{
			\subfigure[Input]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj-2.png}
			}
			\subfigure[L$\alpha\beta$]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj_CIE_2-1.png}
			}
			\subfigure[Harmonization]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj_harmonization_2-1.png}
			}
			\subfigure[Landmark]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj_Landmark_2-1.png}
			}
			\\
			\subfigure[Reference]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj-1.png}
			}			
			\subfigure[NeutralArt]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj_NeutralArt_2-1.png}
			}
			\subfigure[SuperMatch]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj_SuperMatch_2-1.png}
			}
			\subfigure[SuperBig]{
				\includegraphics[height=\height,clip]{./Images/Taj2-1/taj_SuperBig_2-1.png}
			}
		}
	\end{center}
	
	\caption{ Visual comparisons of style transfer among different algorithms.}
	\label{fig:Taj2-1}
\end{figure*}


==> col-2.tex <==

\def\heighto{23mm}
\def\heightt{2.9cm}
\begin{figure*}[htbp]
	\begin{flushright}
		{
			\subfigure[Input]{
				\includegraphics[height=\heighto,clip]{./Images/Taj-1/taj-source_1.png}
			}
            \subfigure[]{
              \begin{overpic}[height=\heighto,clip]{./Images/Taj-1/taj-result-7.png}
                \put(65,34){\includegraphics[height=15mm,clip]{./Images/Taj-1/taj-target7_1.png}}
              \end{overpic}
            }
            \subfigure[]{
              \begin{overpic}[height=\heighto,clip]{./Images/Taj-1/taj-result-8.png}
                \put(65,34){\includegraphics[height=15mm,clip]{./Images/Taj-1/taj-target8_1.png}}
              \end{overpic}
            }
			\\
			\subfigure[]{
              \begin{overpic}[height=\heighto,clip]{./Images/Taj-1/taj-result-10.png}
                \put(65,34){\includegraphics[height=15mm,clip]{./Images/Taj-1/taj-target10_1.png}}
              \end{overpic}
            }
            \subfigure[]{
              \begin{overpic}[height=\heighto,clip]{./Images/Taj-1/taj-result-11.png}
                \put(65,34){\includegraphics[height=15mm,clip]{./Images/Taj-1/taj-target11_1.png}}
              \end{overpic}
            }
		}
	\end{flushright}
	
	\caption{Visual comparisons of SuperBIG style transfer for different reference images.}
	\label{fig:all2}
\end{figure*}


==> step_results.tex <==

\def\height{1.95cm}
\begin{figure*}[htbp]
	\begin{flushright}
		{
			\subfigure[Input]{
				\includegraphics[height=\height,clip]{./Images/step_results/door-source_1.png}
			}
		}
	\end{flushright}
	
	\caption{ Visual comparisons of style transfer among different algorithms.}
	\label{fig:Taj2-1}
\end{figure*}
